PiRank: Scalable Learning To Rank via Differentiable Sorting

A key challenge with machine learning approaches for ranking is the gap between the performance metrics of interest and the surrogate loss functions that can be optimized with gradient-based methods. This gap arises because ranking metrics typically involve a sorting operation which is not differentiable w.r.t. the model parameters. Prior works have proposed surrogates that are loosely related to ranking metrics or simple smoothed versions thereof, and often fail to scale to real-world applications. We propose PiRank, a new class of differentiable surrogates for ranking, which employ a continuous, temperature-controlled relaxation to the sorting operator based on NeuralSort [1]. We show that PiRank exactly recovers the desired metrics in the limit of zero temperature and further propose a divide and-conquer extension that scales favorably to large list sizes, both in theory and practice. Empirically, we demonstrate the role of larger list sizes during training and show that PiRank significantly improves over comparable approaches on publicly available internet-scale learning-to-rank benchmarks.

==> sections/checklist.tex <==
\section{NeurIPS 2021 Paper Checklist}

\begin{enumerate}
    \item \begin{enumerate}
            \item Yes.
            \item Yes.
            \item Yes. See Section \ref{sec:conclusion}.
            \item Yes. See Section \ref{sec:experiments}.
        \end{enumerate}
    \item \begin{enumerate}
            \item Yes. See Appendix \ref{sec:proof}.
            \item Yes. See Appendix \ref{sec:proof}.
        \end{enumerate}
    \item \begin{enumerate}
            \item Yes. See Section \ref{sec:introduction}, Appendix \ref{sec:exp_details}, supplemental material and URL in non-anonymous version.
            \item Yes. See Appendix \ref{sec:exp_details}.
            \item No. We computed error bars for the scale experiments but they are too small to show on the plot (Fig.~\ref{fig:runtime}). However, we did not have adequate compute resources to run benchmark experiments with multiple seeds (Sec.~\ref{sec:benchmark}). Note that the code makes it easy to reproduce the experiments with other seeds (see 3a).
            \item Yes. See Appendix \ref{sec:exp_details}.
        \end{enumerate}
    \item \begin{enumerate}
            \item Yes. See Section \ref{sec:experiments} and Appendix \ref{sec:exp_details}. 
            \item Yes. See Appendix \ref{sec:exp_details}.
            \item Yes. The \name{} code is included.
            \item Yes. The datasets were manually labeled and released by respectively Microsoft for MSLR-WEB30K and Yahoo! for Yahoo! C14.
            \item Yes. They do not. Both datasets are fully anonymized and contain no offensive content.
        \end{enumerate}
    \item Not applicable.
    % \item \begin{enumerate}
    %     \end{enumerate}
\end{enumerate}


